Are We There Yet? Unraveling the State-of-the-Art Smart Contract Fuzzers

Given the growing importance of smart contracts in various applications, ensuring their security and reliability is critical. Fuzzing, an effective vulnerability detection technique, has recently been widely applied to smart contracts. Despite numerous studies, a systematic investigation of smart contract fuzzing techniques remains lacking. In this paper, we fill this gap by: 1) providing a comprehensive review of current research in contract fuzzing, and 2) conducting an in-depth empirical study to evaluate state-of-the-art contract fuzzers' usability. To guarantee a fair evaluation, we employ a carefully-labeled benchmark and introduce a set of pragmatic performance metrics, evaluating fuzzers from five complementary perspectives. Based on our findings, we provide direction for the future research and development of contract fuzzers.

==> backup.tex <==


% % \scalebox{0.9}{
% \begin{table*}[tbh]
% \footnotesize
% %\scriptsize
% \centering
% % \renewcommand{\arraystretch}{0.8}
% % \vspace{-2ex}
% \caption{Table.} 
% \begin{tabular*}
% %{lcccccc}
% {\linewidth}
% {@{\extracolsep{\fill}}r|c|c|c|c|c|c|c}
% %{@{\extracolsep{\fill}}cccccccccc}
% %{\textwidth}
% %{@{\extracolsep{\fill}}lcccccccc}
% \toprule
% \multicolumn{1}{c|}{} &
% \multicolumn{1}{c|}{Problem/Highlight} &
% \multicolumn{2}{c|}{Seed Generation} &
% \multicolumn{3}{c|}{Seed Mutation} &
% \multicolumn{1}{c|}{Seed Scheduling}
% % \multicolumn{3}{c|}{Feedback Mechanism}
% \\
% \cline{1-8}
% % & Single & Sequence & Random & Symbolic &Taint &Heuristic & ML & ABI & Transition & Sequence 
% % & Source & Env
% % & Coverage & Data flow & State\\ 
% &   & Arguments & Sequence &  Argument & Enviroment & Sequence & \\
% \hline

% % Echidna &   &   &   &   &   & 
% % \hline

% ContractFuzzer & \checkmark &   &\checkmark &   &   &   &   &\checkmark  &   &   &   &\checkmark &   &   & \\
% \hline

% \bottomrule
% \end{tabular*}
% % \begin{tablenotes}
% %      \item[1] Seed input: \romannumeral1&) Single: only consider single transaction; \romannumeral2&) Sequence: consider transaction sequence
% %      \item[2] Seed Mutation: \romannumeral1&) ABI: mutate the argumnets in ABI; \romannumeral2&) Transition: like gas price, gas limit;
% %      \romannumeral3&) Sequence: mutate transition(ABI) sequence.
% %      \item[3] Test Oracle: \romannumeral1&) Source: insert Oracles in the source code; 
% %      \romannumeral2&) Env: instrument the environment like EVM to insert Oracles
% %      \item[4] Feedback Mechanisim: \romannumeral1&) Coverage: code coverage ; 
% %      \romannumeral2&) Data flow: e.g. transactions operate on the same contract state variable,
% %      \romannumeral3&)state: contracts’ states.
% % \end{tablenotes}
% \label{table:modelIntegrity}
% \vspace{-3ex}
% \end{table*}


% @{\extracolsep{\fill}}

\begin{table*}[tbh]
\scriptsize
%\scriptsize
\centering
\renewcommand{\arraystretch}{1.3}
\caption{Summary of technical details for existing smart contract fuzzers.}
%\vspace{-2ex}
%\resizebox{\linewidth}{!}{
\begin{tabular*}
%{lcccccc}
{\linewidth}
{@{\extracolsep{\fill}}l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
\hline
% \multirow{2}{*}{\textbf{Tool}}  

\multicolumn{3}{c|}{\textbf{Tool}}&
\multirow{2}{*}{\textbf{G/M}} & 
\multicolumn{6}{c|}{\textbf{Arguments Generation}} 
&\multicolumn{4}{c|}{\textbf{Sequence Generation}}
 &\multicolumn{3}{c|}{\textbf{Seed Mutation}} 
& \multicolumn{3}{c|}{\textbf{Seed Scheduling}}
& \multirow{2}{*}{\textbf{EVM}}

\\
\cline{1-3}
\cline{5-20}
Name & year & OC  &  & Type & Ran & Dict & Prev & ML & Sym & Ran & Dyn & Static & ML & Args & Env & Seq &  Cov & Dis & Bug \\ 
 \hline
 
ContractFuzzer~\cite{jiang2018contractfuzzer} & 2018 &\checkmark & G & \checkmark & \checkmark & \checkmark &   &   &   & \checkmark &   &   &   &   &   &   &   &   &   \\
\hline

Reguard~\cite{liu2018reguard} & 2018 & & M &   & \checkmark &   &   &   &   & \checkmark &   &   &   &  \checkmark  &   &   & \checkmark &   &   \\
\hline

ILF~\cite{he2019learning} & 2019 & \checkmark & G & \checkmark & \checkmark &   &   & \checkmark &   &   &   &   & \checkmark &  \checkmark  & \checkmark &   &   &   &   \\
\hline

SoliAudit~\cite{liao2019soliaudit} & 2019 & \checkmark & G & \checkmark & \checkmark &   &   &   &   & \checkmark &   &   &   & \checkmark & \checkmark &   &   &   &   \\
\hline


ContraMaster~\cite{wang2020oracle} & 2019 & \checkmark & M & \checkmark & \checkmark &   & \checkmark &   &   &  \checkmark &  \checkmark &   &   &  \checkmark & \checkmark & \checkmark & \checkmark &   &   \\
\hline


Harvey~\cite{wustholz2020harvey} &2020 & & M &   & \checkmark &   & \checkmark &   &   & \checkmark &   &   &   & \checkmark  &   &  \checkmark & \checkmark &  \checkmark &   \\
\hline


ETHPlOIT~\cite{zhang2020ethploit} & 2020 & \checkmark & M & \checkmark & \checkmark &   & \checkmark &   &   &   &   & \checkmark &   & \checkmark & \checkmark &   &  \checkmark &   &   \\
\hline


sFuzz~\cite{nguyen2020sfuzz} & 2020 & \checkmark & M &\checkmark  &\checkmark  &   &   &   &   & \checkmark &   &   &   &\checkmark  &\checkmark  &   &  \checkmark &  \checkmark &   \\
\hline

%  mutation????
Echidna~\cite{grieco2020echidna} & 2020 & \checkmark & M & \checkmark & \checkmark & \checkmark  & \checkmark &   &   & \checkmark &   &   &   & \checkmark  &   &   & \checkmark &   &   \\
\hline

GasFuzzer~\cite{ashraf2020gasfuzzer}& 2020 & & M & \checkmark & \checkmark & \checkmark &   &   &   & \checkmark &   &   &   &  \checkmark &   &   &   &   &   \\
\hline


% Tainted
Targy~\cite{ji2021increasing} & 2021 & & M & \checkmark & \checkmark &   &   &   &   & \checkmark &   &   &   &   &\checkmark  &   & \checkmark  & \checkmark  &   \\
\hline


Smartian~\cite{choi2021smartian} & 2021 & \checkmark & M & \checkmark & \checkmark &   &   &   &  \checkmark &   & \checkmark & \checkmark &   & \checkmark & \checkmark &\checkmark  & \checkmark &   &   \\
\hline

SmartGift~\cite{zhou2021smartgift} & 2021 & \checkmark & G & \checkmark & \checkmark &   &   & \checkmark &   & \checkmark &   &   &   &   &   &   &   &   &   \\
\hline

% % Recheck
% taint--->z3 symbolic
ConFuzzius~\cite{torres2021confuzzius} & 2021 & \checkmark & M & \checkmark & \checkmark & \checkmark  &  &   & \checkmark  & \checkmark & \checkmark &   &   & \checkmark & \checkmark & \checkmark & \checkmark &   &   \\
\hline

% % Vulnerable paths
% % Code distance
% data dependency
Beak~\cite{zhang2022beak} & 2022 & & M & \checkmark & \checkmark  & \checkmark   &   &   & \checkmark  &   &   & \checkmark &   & \checkmark & \checkmark & \checkmark &   & \checkmark &  \\
\hline

% static 代表的是什么
xFuzz~\cite{xue2022xfuzz} & 2022 & \checkmark & M &\checkmark  &\checkmark  &   &   &   &   &   &   &\checkmark &\checkmark  &\checkmark  &\checkmark  &   &  \checkmark &  \checkmark &    \\
\hline

EtherFuzz~\cite{wang2022etherfuzz} & 2022 & & M & \checkmark & \checkmark & \checkmark  &   &   &   &\checkmark  &   &   &   & \checkmark & \checkmark & \checkmark & \checkmark &   &    \\
\hline

SmartACE~\cite{wesley2022verifying} & 2022 & \checkmark &M &   & \checkmark &   &   &   &   & \checkmark &   &   &   &   &   &   & \checkmark &   &   \\
\hline

% Constructor followed by callable methods &   &   &   & many-objective
SynTest-S~\cite{olsthoorn2022syntest} & 2022 & \checkmark & M & \checkmark & \checkmark &   &   &   &   & \checkmark  &   &   &   & \checkmark  &   &  \checkmark &   &  \checkmark &    \\
\hline


RLF~\cite{su2022effectively} & 2022 & \checkmark & G & \checkmark & \checkmark &   &   &   &   &   &   &   &  \checkmark & \checkmark & \checkmark &   & \checkmark &   & \checkmark \\
\hline



IR-fuzz~\cite{liu2023rethinking} & 2023 & \checkmark & M & \checkmark & \checkmark &   &   &   &   &   &   & \checkmark &   & \checkmark & \checkmark & \checkmark &   & \checkmark &   \\
\hline

EF\textbackslash CF~\cite{rodler2023ef} &2023 & \checkmark & M & \checkmark  &   & \checkmark  &   &   &   & \checkmark &   &   &   & \checkmark & \checkmark & \checkmark & \checkmark  &   &   \\
\hline

ityfuzz~\cite{shou2023ityfuzz} & 2023 & \checkmark & M & \checkmark & \checkmark & & & & & & & & & & & & \checkmark & & \\

\hline
\end{tabular*}
%}
\label{table:performance2}
\begin{tablenotes}[flushleft]\footnotesize
    \item {\scriptsize In the \textbf{G/M} column, G: generation-based, M: mutation-based;  In the \textbf{Arguments Generation} column, Type: type-awareness, Ran: randomly generated arguments, Dict: arguments from a pre-prepared dictionary, Prev: values previously encountered or used, ML: arguments obtained through machine learning, Sym: arguments obtained via symbolic execution}
    \item {\scriptsize In the \textbf{Sequence Generation} column, Ran: randomly generated transaction sequences, Dyn: sequences generated through analyzing dynamic data flow, Static: sequences generated by analyzing static data flow, ML: sequences generated through machine learning;  In the \textbf{Seed Mutation} column, Args: mutating transaction arguments, Env: mutating environment properties, Seq: mutating transaction sequences; In the \textbf{Seed Scheduling} column, Cov: fitness by coverage, Dis: fitness by distance, Bug: fitness by vulnerability.}
  \end{tablenotes}
%\vspace{-3ex}
\end{table*}

==> tb2.tex <==
\begin{table}[!t]
%\footnotesize
\scriptsize
%\small
%\renewcommand\arraystretch{1.25}
\vspace{-2pt}
\centering
\caption{State-of-the-art smart contract fuzzers.} 
%\vspace{-4pt}
\scalebox{0.8}{
\begin{tabular}{|l|cccc|}
\hline
\textbf{Tool Name}&
\textbf{Year} &
\textbf{Open-source}  &
\textbf{Open-dataset} &
\textbf{Platform}
\\
\hline
\rowcolor{color2}ContractFuzzer~\cite{jiang2018contractfuzzer} & 2018 & $\color{mygreen} \checkmark$ &  $\color{mygreen} \checkmark$ & Ethereum\\
\hline

\rowcolor{color6}Reguard~\cite{liu2018reguard} & 2018 & \color{myred} \ding{55} & \color{myred} \ding{55} & Ethereum\\
\hline

\rowcolor{color2} ILF~\cite{he2019learning} & 2019 &\color{} \ $\color{mygreen} \checkmark$ & \color{myred} \ding{55} & Ethereum\\
\hline

\rowcolor{color6}SoliAudit~\cite{liao2019soliaudit} & 2019 & $\color{mygreen} \checkmark$ & $\color{mygreen} \checkmark$ & Ethereum\\
\hline

\rowcolor{color2}ContraMaster~\cite{wang2020oracle} & 2019 & $\color{mygreen} \checkmark$ & $\color{mygreen} \checkmark$ & Ethereum\\
\hline

\rowcolor{color6}Harvey~\cite{wustholz2020harvey} & 2020 & \color{myred} \ding{55} & \color{myred} \ding{55} & Ethereum\\
\hline

\rowcolor{color2}ETHPlOIT~\cite{zhang2020ethploit} & 2020 & $\color{mygreen} \checkmark$ & \color{myred} \ding{55} & Ethereum\\
\hline

\rowcolor{color6}sFuzz~\cite{nguyen2020sfuzz} & 2020 & $\color{mygreen} \checkmark$ & \color{myred} \ding{55} & Ethereum\\
\hline

\rowcolor{color2}Echidna~\cite{grieco2020echidna,groce2021echidna} & 2020 & $\color{mygreen} \checkmark$ & \color{myred} \ding{55} & Ethereum\\ 
\hline

% \rowcolor{color6}Samreen et al.~\cite{samreen2020reentrancy} & 2020 &\color{myred} \ding{55} &\color{myred} \ding{55} & Ethereum\\
% \hline

\rowcolor{color6}GasFuzzer~\cite{ashraf2020gasfuzzer} & 2020 &\color{myred} \ding{55} & $\color{mygreen} \checkmark$ & Ethereum\\
\hline

\rowcolor{color2}Targy~\cite{ji2021increasing} & 2021 &\color{myred} \ding{55} & $\color{mygreen} \checkmark$  & Ethereum\\
\hline

% \rowcolor{color6}echidna-parade~\cite{groce2021echidna}  & 2021 & $\color{mygreen} \checkmark$  & \color{myred} \ding{55} &  Ethereum \\
% \hline

% echidna-parade & 2020 &  & \\ 
% \hline

\rowcolor{color6}Smartian~\cite{choi2021smartian} & 2021 & $\color{mygreen} \checkmark$ & $\color{mygreen} \checkmark$ & Ethereum\\ 
\hline

\rowcolor{color2}SmartGift~\cite{zhou2021smartgift} & 2021 & $\color{mygreen} \checkmark$  & $\color{mygreen} \checkmark$ & Ethereum \\
\hline

\rowcolor{color6}ConFuzzius~\cite{torres2021confuzzius} & 2021 & $\color{mygreen} \checkmark$ & $\color{mygreen} \checkmark$  & Ethereum \\
\hline

\rowcolor{color2}Beak~\cite{zhang2022beak} & 2022 & \color{myred} \ding{55} & \color{myred} \ding{55} & Ethereum\\
\hline

\rowcolor{color6}xFuzz~\cite{xue2022xfuzz}  & 2022 & $\color{mygreen} \checkmark$ & $\color{mygreen} \checkmark$ & Ethereum\\
\hline

\rowcolor{color2}EtherFuzz~\cite{wang2022etherfuzz} & 2022 & \color{myred} \ding{55} & \color{myred} \ding{55} & Ethereum \\
\hline


\rowcolor{color6}SmartACE~\cite{wesley2022verifying} &  2022 & $\color{mygreen} \checkmark$  & $\color{mygreen} \checkmark$ & Ethereum \\
\hline


\rowcolor{color2}SynTest-Solidity~\cite{olsthoorn2022syntest} & 2022 & $\color{mygreen} \checkmark$ & $\color{mygreen} \checkmark$  & Ethereum \\
\hline

\rowcolor{color6}RLF~\cite{su2022effectively} & 2022 & $\color{mygreen} \checkmark$ & \color{myred} \ding{55} & Ethereum\\
\hline

\rowcolor{color2}effuzz~\cite{ji2023effuzz} & 2023 &  \color{myred} \ding{55} &  \color{myred} \ding{55} & Ethereum\\
\hline


\rowcolor{color6}IR-fuzz~\cite{liu2023rethinking} & 2023 & $\color{mygreen} \checkmark$  & $\color{mygreen} \checkmark$ & Ethereum\\
\hline

\rowcolor{color2}EF\textbackslash CF~\cite{rodler2023ef} & 2023 & $\color{mygreen} \checkmark$ &$ \color{mygreen} \checkmark$ & Ethereum\\
\hline

\rowcolor{color6}ityfuzz~\cite{shou2023ityfuzz} & 2023 & $\color{mygreen} \checkmark$ &$ \color{mygreen} \checkmark$ & Ethereum\\
% \hline
% \bottomrule

% \rowcolor{color6}Effuzz~\cite{ji2023effuzz} & 2023 & \color{myred} \ding{55} & \color{myred} \ding{55} & Ethereum\\
% \hline

% \rowcolor{color2}EOSFuzzer~\cite{huang2020eosfuzzer}  & 2021  & $\color{mygreen} \checkmark$ & $\color{mygreen} \checkmark$ & EOSIO \\
% \hline

% \rowcolor{color6}HFContractFuzzer~\cite{ding2021hfcontractfuzzer} & 2021 & \color{myred} \ding{55} & $\color{mygreen} \checkmark$ & Hyperledger \\
% \hline

% \rowcolor{color2}AntFuzzer~\cite{zhou2022antfuzzer}  & 2022 & \color{myred} \ding{55} & \color{myred} \ding{55} & EOSIO\\
% \hline

% \rowcolor{color6}WASAI~\cite{chen2022wasai}  & 2022 & $\color{mygreen} \checkmark$  & $\color{mygreen} \checkmark$ & WebAssembly\\


\hline
\end{tabular}
}
\vspace{-4pt}
\label{table:scope}
\end{table}

